Whitepaper on Reusable Hybrid and Multi-Cloud Analytics Service Framework

Over the last several years, the computation landscape for conducting data analytics has completely changed. While in the past, a lot of the activities have been undertaken in isolation by companies, and research institutions, today's infrastructure constitutes a wealth of services offered by a variety of providers that offer opportunities for reuse, and interactions while leveraging service collaboration, and service cooperation. This document focuses on expanding analytics services to develop a framework for reusable hybrid multi-service data analytics. It includes (a) a short technology review that explicitly targets the intersection of hybrid multi-provider analytics services, (b) a small motivation based on use cases we looked at, (c) enhancing the concepts of services to showcase how hybrid, as well as multi-provider services can be integrated and reused via the proposed framework, (d) address analytics service composition, and (e) integrate container technologies to achieve state-of-the-art analytics service deployment

==> section/definitions.tex <==
\FILE{section-definitions.tex}

\section{Definitions and Concepts}
\label{sec:definitions}

In this section we provide a list of definitions and doncepts that
help communication between different interdisciplinary groups while
allowing them to use the same language.

A comprehensive glossary (Appendix \ref{sec:glossary}) is provided in the appendix. 

\begin{description}

\item[Analytics Service] 

\item[Analytics Catalog]

\item[Analytics Registry]

\item[Analytics Workflow]

\item[Payload]

\item[Analytics:] The systematic analysis of data, to uncover patterns and relationships between data,
historical trends, and attempts at predictions of future behaviors and events.

\item[Analytics management:] A sub function within the [metadata] registry.
Analytics services azure cognitive, google analytics, aws [dozens], watson analytics... in contrast
to ML frameworks like tensorflow, pytorch, caffe2, and in contrast to Programming libraries
like python, scikit, shiny, or R Studio [??]

\item[Analytics Workflow:] The sequence of processes or tasks part of the analysis


\end{description}



==> section/glossary.tex <==
\FILE{section-glossary.tex}

\section{Glossary}
\label{sec:glossary}

\TODO{remove all terms that are not used or are important.}

This Glossary provides terms that are used in this document. In
addition we have provided a definitions in Section \ref{sec:defining}
to focus on the details of some terms and terminology used in this
document specifically focus sing on Analytics Services.

\begin{description}

  
\item[AAI:] Authentication and Authorization
  Infrastructure. Facilitates single, virtualized identities (issued
  by the {\em user's home organization.})

\item[AARC:]   \TODO{Russell: The Authentication and Authorisation for
  Research and Collaboration project. I will write a descriptive
  sentence for it that you can add later. Also, below, ACL: access
  control list? I have a bunch other acronyms with descriptions that I
  can just send you as a list that you can choose from and add if you
  wish. Under Iaas, p is probably referring to PaaS}  

\item[ABAC:] attribute based access control

\item[ACL:] \TODO{Russell}{TBD}

\item[ACID:] Atomicity, Consistency, Isolation, Durability.

\item[Analytics:] The systematic analysis of data, to uncover patterns
  and relationships between data, historical trends, and attempts at
  predictions of future behaviors and events.

\item[Analytics management:] A sub function within the [metadata]
  registry.

\item[Analytics services] azure cognitive, google analytics, aws
  [dozens], watson analytics... in contrast to ML frameworks like
  tensorflow, pytorch, caffe2, and in contrast to Programming
  libraries like python, scikit, shiny, or R Studio [??]


\item[Analytics Workflow:] The sequence of processes or tasks part of
  the analysis

\item[API:] Application Programming Interface

\item[ASCII:] American Standard Code for Information Interchange

\item[BASE:] Basically Available, Soft state, Eventual consistency
  Classification scheme per 11179, a container of the classifiers for
  all kinds of administered items including common data elements
  [CDE]s.

\item[CIA:] Confidentiality, Integrity, and Availability.

\item[CLI:] Command Line Interface.

\item[Consumer:] Ametadata consumer, per IHE, is responsible for the
  import of metadata created by the source. In the context of section
  A.3,

\item[Container:] See
  \url{http://csrc.nist.gov/publications/drafts/800-180/sp800-180_draft.pdf}
  Cloud Computing The practice of using a network of remote servers
  hosted on the Internet to store, manage, and process data, rather
  than a local server or a personal computer. See
  \url{http://nvlpubs.nist.gov/nistpubs/Legacy/SP/nistspecialpublication800-145.pdf}.

\item[CDE:] Common data element = smallest meaningful data container
  in a given context.

\item[DDC:] data dictionary component. library of data elements that
  are used to establish common understanding of the meaning of coding
  systems.

\item[Data element:] Describes [or defines] the logical unit of
  data. Per 11179, the element refers to the structure of the data,
  distinct from a data instance.

\item[Data element concept:] the combination of an object class, and a
  related property.

\item[DEX:] Data element exchange = interoperability profile. Enables
  retrieval of extraction specifications for data elements which are
  defined in particular domains. ``Options'' including the cross
  enterprise doc sharing [XDS] doc type binding option and the cross
  community access [XCA] doc type binding option, extend basic DEX
  functionality, addressing interoperability with Secondary Data
  Usage[s]. Allowing secondary users to know if and where [data] is
  available when it is organized as a doc sharing environment,
  I.e. XDS, MPQ, XCA.

\item[DevOps:] A clipped compound [?] [portmanteau?] of software
  DEVelopment and information technology OPerationS \TODO{improve}

\item[Deployment:] The action of installing software on resources

\item[DMTF:] Distributed Management Task Force. A standards
  organization.

\item[Extraction Specification:] a map of data locations used as a
  guide for extracting data. SPARQL, SQL, and XPath scripts, aka
  mapping scripts, are examples of specifications for locating a data
  element in a particular content model.

\item[FIM:] federated identity management. A core component of AAI.


\item[Federated database system:] two definitions: 1. a system that
  maps multiple autonomous database systems using a combining scheme
  where one DB interface is provided for local / owner access to data,
  and another simpler interface is provided for guest access to non
  owner data. 2. a DBMS which is an element of a federated group, that
    allows members belonging to the same federated group, to access
    data residing in the DBMS.

\item[HTTP:] HyperText Transfer Protocol HTTPS HTTP Secure

\item[Hybrid Cloud:] See
  \url{http://nvlpubs.nist.gov/nistpubs/Legacy/SP/nistspecialpublication800-145.pdf}.


\item[IaaS:] Infrastructure as a Service SaaS Software as a Service
  Implementation.

\item[IGTF:] Interoperable Global Trust Federation.

\item[ITL:] Information Technology Laboratory metadata data employed
  to annotate other data with descriptive information.

\item[IHE:] \TODO{Russel, TBD}

\item[LDAP:] Lightweight Directory Access Protocol. A
  directory/registry standard.

\item[Metadata generator:] A sub function within the repository
  Metadata Registry [MDR] a database that manages the semantics of
  data elements, and this case, provides discovery and analytics
  management services.

\item[MRR:] Metadata registry / repository = specialized DB of
  metadata which describe data constructs.

\item[Microservice:] Architecture Is an approach to build applications
  based on many smaller modular services. Each module supports a
  specific goal and uses a simple, well-defined interface to
  communicate with other sets of services.

\item[NBDIF] \TODO{}{TBD}
  
\item[NBD-PWG:] NIST Big Data Public Working Group.

\item[NBDRA:] NIST Big Data Reference Architecture.

\item[NBDRAI:] NIST Big Data Reference Architecture Interface.

\item[NIEM:] National information exchange model = government wide
  standards based approach to exchanging information in the US.

\item[NIST:] National Institute of Standards and Technology.

\item[OGF:] Open Grid Forum.

\item[OS:] Operating System.

\item[P2P:] Peer to Peer.

\item[PKI:] Public Key Infrastructure. a security related certificate
  aka X.509.

\item[Proxy:] \TODO{}{TBD}

\item[Registry:] \TODO{}{TBD}
  
\item[Registry, federated:] \TODO{}{TBD}


\item[REST:] REpresentational State Transfer Retrieval a transaction
  where a system returns a selection I.e. a list of data elements from
  a database, or in the scope of this document, a list of elements in
  a metadata registry.

\item[SAML:] Security assertion markup language. a security standard;
  web browser service that defines ``syntax and semantics to exchange
  auth and auth data between security domains.'' Not compatible with
  other authentication protocols such as Secure socket?, OIDC, etc.

\item[Serverless Computing:] Serverless computing specifies the
  paradigm of function as a service (FaaS). It is a cloud computing
  code execution model in which a cloud provider manages the function
  deployment and utilization while clients can utilize them. The
  charge model is based on execution of the function rather than the
  cost to manage and host the VM or container.

\item[Services:] \TODO{TBD}

\item[Service registry:] in the context of an SOA architecture, this
  registry is a network based directory that contains available
  services.

\item[Software stack:] A set of programs and services that are
  installed on a resource to support applications.  Value domain the
  description of a permissible set of values for the property of a
  data element definition.

\item[XACML] eXtensible Access Control Markup Language. a security
  related standard developed by OASIS, circa 2005.

\end{description}




==> section/interfaces.tex <==
\FILE{section-interfaces.tex}

\subsection{Analytics Interfaces}
\label{sec:interfaces}


==> section/introduction.tex <==
\FILE{section-introduction.tex}

\newcommand{\WG}{\TODO{Wo: define name of wrking group}{WORKINGGROUP}}

\section{Introduction}


\subsection{Background}

\TODO{add related research section here}

Keywords:

* cloud

* rest services

* microservices

* hybrid

* fair

* analytics as a service

* software as a service

* data analytics as a service

* data mining

* computation

* descriptive analytics to describe and summarize information from data

* function analytics

* machine learning integration


\subsection{Scope and Objectives}

NBD-PWG\footnote{\TODO{introduce in the background section. THe
background section has been integrated here. check valitity and fix
somehow.}} is exploring how to extend
NBDIF \footnote{\TODO{introduce in the background section. THe
background section has been integrated here. check valitity and fix
somehow.}} for packaging scalable analytics as services to meet the
challenges of today's information analytics. These services are
intended to be reusable, deployable, and operational for Big Data,
High Performance Computing, AI machine learning (ML), and deep
learning (DL) applications, regardless of the underlying computing
environment.

This document explores key focus areas and document level of interest
from industry, government, and academia in extending the NBDIF to
develop scalable analytics as services that are reusable, deployable,
and operational, regardless of the underlying computing environment.
\TODO{Russel: note that the 'string' reusable, deployable, and
  operational was also used in the previous ppg.}


The work has been conducted with input from the NIST BIg Data Working
group while enhancing their original activities to address
requirements for Analytics Service. This includes hosted on
computational resources including Clouds, Containers, and High
Performance Computing (HPC), thus targeting analytics services hosted
on premis, private and public clouds. We have chosen REpresentational
State Transfer (REST) to formulate some details of the architecture,
it is independent from REST and can be formulated in other
frameworks. While using REST we use a familiar pattern for architect,
implementer, and strategists. Due to the many frameworks, programming
languages and services supporting REST the architecture can easily be
enhanced and implemented with various technical solutions.


TBD:

The
analytics framework also targets big data.
Big data is a term used to
describe extensive datasets, primarily in the characteristics of
volume, variety, velocity, and veracity. While opportunities exist
with Big Data analytics, the data characteristics can overwhelm
traditional technical approaches, and the growth of data is outpacing
scientific and technological advances in data analytics.

To advance
progress in Big Data analytics, the NIST Big Data Public Working Group
(NBD-PWG) is working to develop consensus on important fundamental
concepts related to Big Data. The results are reported in the NIST Big
Data Interoperability Framework (NBDIF) series of volumes.



==> section/outreach.tex <==
\FILE{section-outreach.tex}

\section{Outreach}
\label{sec:outreach}

TBD


==> section/production.tex <==
\FILE{section-production.tex}

\newcommand{\WG}{OUR WORKING GROUP}

\section*{Report Production}


This document is conducted as part of the NIST \WG. The working group
holds public meetings regularly Tuesdays at 1 pm. The
working group is public, and anyone can join that is interested in
contributing to this document and bringing it to completion. We will
be using GitHub to coordinate this work. Although the work is done in
a public working group, we had one member of the group asking to keep
the document private. As such, you need to join our meeting group first
before we grant you access to this document. You can join the working
group by contacting Wo Chang at \href{mailto:wchang@nist.gov}{wchang@nist.gov}.


The production of this document is conducted to address the following
needs

\begin{enumerate}
  \item a one-page executive summary, 

  \item a detailed specification,

  \item use cases that support this document that may be hosted in
    separate documents. Such documents could follow the template as
    provided at \cite{nist-bigdatawg}.

\end{enumerate}


\parindent0pt We are using the following tools to manage the completion of
the document:

\begin{itemize}

\item
  \href{https://www.overleaf.com/project/619ba513e4aade4400e06df8}{an
    online document $\rightarrow$} we work on in Overleaf. Oevrleaf
  sinks to GitHub are done however only on a best effort basis. SO
  before you start working, make sure you pull in overleaf from
  GitHub.

\item \href{https://github.com/cyberaide/NIST-analytics/projects/1}{a task list
  $\rightarrow$} in GitHub,

\item \href{https://github.com/orgs/cyberaide/}{a versioned document
  source $\rightarrow$} in GitHub,

\item \href{https://nist-analytics.slack.com}{a slack channel
  $\rightarrow$} to increas the communication outside of the Working
  group meetings and to coordinate task.

\item
  \href{https://github.com/cyberaide/NIST-analytics/raw/main/NIST-analytics.pdf}{a
    regularly updated PDF document} with editing links pointing to the
  GItHub versioned documents. Please note that for the most recent
  document you will have to use GitHub or Overleaf. 
  
\end{itemize}

Once you have joined the Working group, you can get access to the
document directories by contacting \href{mailto:laszewski@gmail.com}{laszewski@gmail.com}.

\begin{quote}

{\em Please note that we stopped using Word for the document
  management contributors consistently used different templates and
  formatting rules resulting in unsustainable multi hourlong cleanups
  every week instead of being able to focus on content. For this
  reason, we will not switch back to Word. However, a section could be
  written in markdown, which can easily be integrated into the
  document. Formatting should be kept at a minimum.}

\end{quote}


\subsection*{Annotations}

It is easy to anotate content in the document we use the following,
while the person specified is supposed to fix it: \\

\TODO{Gregor: The issue we observe}

\begin{verbatim}
\TODO{Gregor: The issue we observe}
\end{verbatim}

If a person name is not specified anyone is encouraged to fix
it. Todos will beintgrated in a list of todos that are included at the
end of the document in an appendix

We also use comments that are not included in the todolist, but may
serve as temprary visual aides to alert, highlight or anotate
text. This includes \\

\begin{tabular}{ll}
\verb|\alert{Please address this}| & \alert{Please address this} \\
\verb|\highlight{a highight}| & \highlight{a highight} \\
\verb|\add{add this text}| & \add{add this text} \\
\verb|\remove{remove this text}| & \remove{remove this text} \\
\verb|\replace{old text}{with new text}| & \replace{old text}{with new text} \\
\end{tabularr}



==> section/resources.tex <==

\subsection{Resource Management}
\label{sec:resources}

Here we investigate and define a minimal set of resource management
services and interfaces for application orchestration and workflow
between processes.


==> section/reusability.tex <==
\FILE{section-reusability}
\section{Reusable Analytics Services}

The main section include the definition and conceptual
architecture of reusable analytics services.


\input{section-registry}

\input{section-data}

\input{section-security}

\input{section-packaging}

\input{section-resource-management}







==> section/section-nlp.tex <==
\FILE{section-nlp.tex}

\section{NLP}


Natural Language Processing was one of the first services offered by
many cloud providers. This was motivated by analyzing large amounts of
text in volume and number and deriving automated content from
it. Popular services include keyword extraction, sentiment analysis,
auto summary, and translation.  The services are offered often by large
cloud providers such as Google, IBM Watson and Amazon to consumers for
a fee. In addition such tools are also offered as stand alone
components and software packages.

As many such services are offered by the different providers, and
standalone components and software packages exist, it allows us to use
them to test the framework for implementing hybrid and multi-cloud
analytics services. We can therefore analyze each of their APIs and
compare functionality as well as the performance characteristics of
local as well as cloudservices. We also can test our design of the
cloud service catalog to identify the strategy of dynamically
locating similar services and integrate them into a service offering.

For our work we have restricted our analysis to two cloud services
from Amazon ans Google, while the integration of a third from Amazon
is under development. Furthermore we have only considered the
translation service as it provides an easy abstraction of a service
that translates a text from a source language to a target langauge:

\begin{Verbatim}[fontsize=\small]
def translate(text, source_langauge, target_langauage, ...):
    ...
    return translation
\end{Verbatim}

Each of the services is implemented with a different API. We contrast
the API in Figure ... showcaseing the difference in invoking a
translation service as well as showcasing the result of the json
response of such a service.


If the interface is on purpose defined differently a switch will cost
extra work and may therfore not be in the interest of the users.  It
is obvious that users can benefit from a uniform implementation of
this API in order to easily switch from one provider to the other.
Naturally the cloud providers typically do not have any interrest in
providing such a uniform API as it may entise the customers to switch
service providers.

Hence a multicloud CLI implementation may look as followes, where the
provider flag is used to distinguish the different cloud providers
offering the translation service. Naturally, we could also utilize a
local translation program such as offered from ... and easily make
this example a hybrid service that also integrates with a local
implementation.


\begin{Verbatim}[fontsize=\small]
cms nlp translate --provider=google --from=en --to=de hello world
cms nlp translate --provider=aws --from=en --to=de hello world
cms nlp translate --provider=local --from=en --to=de hello world
\end{Verbatim}


As eachof the services returns natively a different outout, it is
beneficial to unify the output and create a mapping from the
originating service to the output. An example for such a uniform output is given next.
ml          

\begin{Verbatim}[fontsize=\small]
{'date': '05/02/2022 14:45:45',
 'input': 'hello world',
 'input_language': 'en',
 'output': 'Hallo Welt',
 'output_language': 'de',
 'provider': 'aws',
 'time': 0.2641}
\end{Verbatim}


Other parameters such as service region can easily be integrated in
this example. Furthermore, it is obvious that the commandline
application underlaying API can be used in a REST service
implementation and can be generalized into different REST service
frameworks. For our implementation we have used FastAPI and used the
closest regional service center to our location.

The result of the translation that simply translates a text from
German ``Hallo Welt'' to English ``Hello World'' is showcased for 100
invocations in Figure~\ref{fig:translate}. 

\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=1.0\columnwidth]{images/nlp-helloworldbenchmark.pdf}
    \end{center}
  \caption {Architecture of the hybrid multi-analytics service
    framework}
  \label{fig:translate}
\end{figure}

Such a performance analysis could be performed based on customer needs
and could indicate factors for preferential service choices. THis may
include besides time other factors such as cost and qaulity, or even
service level reliability at different times.

For us we found that in for the short query we used the service
offered by AWS to translate the text was on average ...  seconds
faster when executed from Bloomington, IN to the closest service
centers for the providor.





==> section/talk.tex <==

\section{Talk}

\textit{Reusable Hybrid and Multi-Cloud Analytics Service Framework}
Gregor von Laszewski (laszewski@gmail.com),
University of Virginia, 
Charlottesville, VA, USA

Over the last several years, the computation landscape for conducting 
data analytics has completely changed. While in the past,
a lot of the activities have been undertaken in isolation by companies,
and research institutions, today's infrastructure constitutes a wealth
of analytics services offered by a variety of providers that offer opportunities
for reuse, interactions while leveraging service collaboration, and service cooperation.

In this talk, we project our vision to develop an analytics services framework to integrate reusable hybrid multi-services across different cloud infrastructure and service providers as well 
as on-premise infrastructure and services. It includes (a) analytics services that explicitly target the intersection of hybrid multi-provider analytics services, (b) the integration of sensor networks into the service data, (c) the integration of advanced modeling services as part of analytical tasks such as earthquake prediction, and (d) the coordination of these services. We showcase how our vision can integrate leveraging service composition with cooperation and competition analytics services. We demonstrate the activities while utilizing benchmark analytics services as used by the  MLCommons science benchmark working group.

==> section/ufo.tex <==
\subsection{Scope and Objectives}

NBD-PWG\footnote{\TODO{introduce in the background section. THe
background section has been integrated here. check valitity and fix
somehow.}} is exploring how to extend NBDIF \footnote{\TODO{introduce
in the background section. THe background section has been integrated
here. check valitity and fix somehow.}} for packaging scalable
analytics as services to meet the challenges of today's information
analytics. These services are intended to be reusable, deployable, and
operational for Big Data, High Performance Computing, AI machine
learning (ML), and deep learning (DL) applications, regardless of the
underlying computing environment.

This document explores key focus areas and document level of interest
from industry, government, and academia in extending the NBDIF to
develop scalable analytics as services that are reusable, deployable,
and operational, regardless of the underlying computing environment.
\TODO{Russel: note that the 'string' reusable, deployable, and
  operational was also used in the previous ppg.}


The work has been conducted with input from the NIST BIg Data Working
group while enhancing their original activities to address
requirements for Analytics Service. This includes hosted on
computational resources including Clouds, Containers, and High
Performance Computing (HPC), thus targeting analytics services hosted
on premis, private and public clouds. We have chosen REpresentational
State Transfer (REST) to formulate some details of the architecture,
it is independent from REST and can be formulated in other
frameworks. While using REST we use a familiar pattern for architect,
implementer, and strategists. Due to the many frameworks, programming
languages and services supporting REST the architecture can easily be
enhanced and implemented with various technical solutions.


TBD:

The
analytics framework also targets big data.
Big data is a term used to
describe extensive datasets, primarily in the characteristics of
volume, variety, velocity, and veracity. While opportunities exist
with Big Data analytics, the data characteristics can overwhelm
traditional technical approaches, and the growth of data is outpacing
scientific and technological advances in data analytics.

To advance
progress in Big Data analytics, the NIST Big Data Public Working Group
(NBD-PWG) is working to develop consensus on important fundamental
concepts related to Big Data. The results are reported in the NIST Big
Data Interoperability Framework (NBDIF) series of volumes.



==> usecase/health.tex <==
\subsection{Health care}

\Data Analytics as a service holds great promise for more accurate healthcare diagnostics and even prediction of disease outcomes for patients. 
 
A-Critical Care Diagnoses
Data analytic and ML tools to help prevent overcrowding in the hospital unit. Research has shown that patients coming to the hospital with a particular type of heart attack did not require hospitalization in the ICU. By enhancing the medical informatics analytic as a service, Emergency Room (ER) clinicians identify these patients and refer them to noncritical care. This service would improve the quality of care for patients and reduce unnecessary costs—high Rick stable patients with Non-ST-Segment-Elevation.
In the United States, ≈40% of patients with non–ST-segment–elevation myocardial infarction (NSTEMI) who initially present without cardiogenic shock or cardiac arrest is admitted to the intensive care unit (ICU). ICU utilization for these initially stable NSTEMI patients varies substantially between care providers. 
The severity of illness on presentation is similar for NSTEMI patients treated and not treated in the ICU. Therefore risk-based ICU utilization—admitting those at the highest risk of developing complications requiring ICU care to the ICU and admitting those at lower risk to a non-ICU setting—has the potential to align resource use with patient needs.
For patients with initially stable NSTEMI, the Acute Coronary Treatment and Intervention Outcomes Network (ACTION) ICU risk score uses data available at the time of hospital presentation to predict the risk of clinical deterioration requiring ICU care— in-hospital death, cardiac arrest, shock, respiratory failure, heart block requiring pacemaker placement, and stroke. Risk scores are infrequently used in clinical practice, but embedding a risk score calculator with associated decision support into the electronic 
health records (EHR) could increase uptake. 
 
 B- Radiology
Imaging methods include computed tomography (CT), magnetic resonance imaging (MRI), and X-ray, offering analytic/computational capabilities that process images with incredible speed and accuracy. Recognizes complex patterns to assess a patient's health, even predictions of disease outcomes for patients. However, sophisticated analytic as a service needs more robust evaluation methods to reduce risk to the patient, establish trust, and ensure wider adoption. A clear example is many researchers' difficulty in classifying imaging results from early studies of the coronavirus disease that spawned the COVID-19 pandemic.



TODO{This section does not include how analytics services are used and we use it}

A technician in the hospital uses voice commands to control an MRI
machine to take tomographic images. The images will be automatically
sent to a private analytics service to identify if the images contain
signs of COVID-19. In this case. multiple services are consulted to
assure that the best available and appropriate algorithms are chosen.
Once identified, an image can be sent to a public analytics service
(given patient consent).

\TODO{the following ppg needs more than editing}

In order to improve the available images to improve the deep learning
data analysis. Previous images that have tested negative may be
reanalyzed with the newly improved models. If new cases are found
based on the improved analysis, health care providers are notified,
and further actions regarding the treatment plan by the supervising
physician is cast. As we can see, this example has all the ingredients
that we need to create a new generation of services that integrates
on-premise infrastructure, public and private services. The
orchestration of the services as well as a convenient
interface. Automation of the workflow of this use case example is
explicitly stated.

Analyzing this example, we identify a mixture of services that utilize
on-premise infrastructure (the MRI), private and public services. A
variety of service patterns are used in concert to establish an analysis
pipeline targeted explicitly for this application use case. 

The goal of this work is to analyze the interoperability of such
service scenarios and identify such patterns motivating a vendor
neutral architecture that promotes reusable implementations to 
support aspects of similar use cases addressed by them.


This use case has the implict requirements needing the following
aspects to be addressed by the framework we develop.

\begin{enumerate}

\item{\bf AS vendor neutral cloud and computer service integration.} ...

  \begin{enumerate}
  \item {\bf AS in cloud.} ...
  \item {\bf AS in LCCF.} ...
  \item {\bf AS in microservices.} ...
  \end{enumerate}

\item{\bf AS architecture.} ...

  \begin{enumerate}
  \item{\bf AS vendor neutral interfaces.} ...
  \item{\bf AS REST.} ...
  \item{\bf AS layers such as interface, service layer, and provider layer.} ...
  \end{enumerate}

\item{\bf AS workflow.} ...

  \begin{enumerate}
  \item{\bf AS catalog and registry.} ...
  \item{\bf AS cooperation.} ...
  \item{\bf competition.} ...
  \item{\bf AS orchestrator.} ...
  \end{enumerate}


\item{\bf AS calculation.}

  \begin{enumerate}
  \item{\bf AS with DL.} ...
  \item{\bf AS data analytics.} ...
  \end{enumerate}

\item{\bf AS security.} ...

\end{enumerate}




==> usecase/weather.tex <==
\FILE{usecase/weather.tex}
\subsection{Use Case: Numeric Weather Prediction}

\TODO{This section does not include lessons learneed and summarizes which analytics services we need.}

\paragraph*{Background.} Large amounts of weather data ar e produced continually and stored in
many different databases.  Accurate weather predictions require large
amount s of processing power to accurately simulate conditions
worldwide at a high resolution and fre quent intervals. One of the
most computationally consuming parts of a reliable weather model is th
e microphysics scheme. The current microphysics scheme, Weather
Research and Forecasting (WRF) Single Moment 6-class Microphysics
(WSM6), simulates the processes in the atmosphere that leadto the
formation and precipitation of rain, snow, and graupel and requires
complex floating-point operations needing to be performed on vast
amounts of data for accurate simulations. As computer
performanceimproves, so does the Numerical Weather Prediction (NWP)
models' resolution and accuracy. However, there is still much progress
to be made, as simulation accuracy still falls off sign ificantly for
predictions more than 36 hours in advance. Figure \ref{fig:weather-1}
shows the general WRF modeling system flow chat.

\begin{figure}[htb]
\centering\includegraphics[width=1.0\columnwidth]{usecase/nwp-arch.png}
\label{fig:weather-1}
\caption{WRF Modeling System Flow Chart with Various Configuration.} 
\end{figure}

\paragraph*{Functionalities and Activities} (based on Big Data Application Provider of NBDIF Ref. Architecture).
In this case study, we only focus on two main functionalities, namely
WPS and WRF, and their activities.  Figure \ref{fig:weather-2} shows
the cross-functional diagram for their actions.

WPS Activities:

\begin{figure}[htb]
\centering\includegraphics[width=1.0\columnwidth]{usecase/weather.png}
\label{fig:weather-2}
\caption{Cross-Functional Diagram Numerical Weather Prediction.}
\end{figure}

\begin{enumerate}
  
\item geogrid -- defines simulation domains and interpolate various terrestrial data sets to the
model grids. Input data available at [1].

\item ungrib -- extracts needed meteorological data and packs it into an intermediate file format.
Input data available at [2]

\item medgrid -- prepares horizontally interpolate the meteorological data onto the model domain.
  Input data from the output of geogrid and ungrib.

\end{enumerate}

WRF Activities:

\begin{enumerate}

\item real -- prepares vertically interpolates the output from metgrid, and creates a boundary and initial
condition files with some consistency checks.

\item wrf -- generates a model forecast.

\end{enumerate}

\paragraph*{Datasets.}

\begin{enumerate}
  
\item WRF Users Page, WPS V4 Geographical Static Data Downloads Page \cite{wrf-data}

\item NCEP FNL Operational Model Global Tropospheric Analyses, continuing
from July 1999 \cite{cisl_rda_ds083.2}

\end{enumerate}


This use case has the implict requirements needing the following
aspects to be addressed by the framework we develop.

\begin{enumerate}

\item{\bf AS vendor neutral cloud and computer service integration.} ...

  \begin{enumerate}
  \item {\bf AS in cloud.} ...
  \item {\bf AS in LCCF.} ...
  \item {\bf AS in microservices.} ...
  \end{enumerate}

\item{\bf AS architecture.} ...

  \begin{enumerate}
  \item{\bf AS vendor neutral interfaces.} ...
  \item{\bf AS REST.} ...
  \item{\bf AS layers such as interface, service layer, and provider layer.} ...
  \end{enumerate}

\item{\bf AS workflow.} ...

  \begin{enumerate}
  \item{\bf AS catalog and registry.} ...
  \item{\bf AS cooperation.} ...
  \item{\bf competition.} ...
  \item{\bf AS orchestrator.} ...
  \end{enumerate}


\item{\bf AS calculation.}

  \begin{enumerate}
  \item{\bf AS with DL.} ...
  \item{\bf AS data analytics.} ...
  \end{enumerate}

\item{\bf AS security.} ...

\end{enumerate}



